Phenomenology of Left-Right Models in the quark sector

A natural avenue to extend the Standard Model (SM) is to embed it into a more symmetric framework. Here, I focus in Left-Right (LR) Models, which treat left- and right-handed chiralities on equal footing. Important information about the structure of LR Models comes from meson-mixing observables. Due to the impact of the new contributions to these processes, I consider the calculation of the short-distance QCD effects correcting the LR Model contributions to meson-mixing observables at the Next-to-Leading Order. I then revisit the phenomenology of a simple realization of LR Models, containing doublet scalars, and combine in a global fit electroweak precision observables, direct searches of the new gauge bosons and meson oscillation observables, a task performed within the CKMfitter statistical framework. Finally, I also cover a different issue, namely the modeling of theoretical uncertainties, a class of uncertainties specially important for flavour physics. Different frequentist schemes are compared, and their differences are illustrated with flavour-oriented examples.

==> Abstract.tex <==
\begin{center}
{\bf {\Large Phenomenology of Left-Right Models in the quark sector } }

\vspace{0.5cm}

{\renewcommand{\thefootnote}{\fnsymbol{footnote}}
%Luiz Vale Silva$^{a,b,}$
Luiz Vale Silva\footnote[1]{PhD advisors: Sébastien Descotes-Genon and Véronique Bernard.}\footnote[2]{luiz.vale@th.u-psud.fr, vale.henrique@ijs.si}
}

\vspace{0.2cm}

\emph{Laboratoire de Physique Th\'eorique (UMR 8627), CNRS, Univ. Paris-Sud,\\ Universit\'e Paris-Saclay, 91405 Orsay Cedex, France}\\
\emph{Groupe de Physique Th\'eorique, Institut de Physique Nucl\'eaire (UMR 8608),\\ CNRS/IN2P3, Univ. Paris-Sud, Universit\'e Paris-Saclay, 91406 Orsay Cedex, France}

\vspace{3\baselineskip}

\vspace*{0.5cm}
%
\textbf{Abstract}\\
%
\vspace{1\baselineskip}
%
\parbox{0.9\textwidth}{A natural avenue to extend the Standard Model (SM) is to embed it into a more symmetric framework. Here, I focus in Left-Right (LR) Models, which treat left- and right-handed chiralities on equal footing. Important information about the structure of LR Models comes from meson-mixing observables. Due to the impact of the new contributions to these processes, I consider the calculation of the short-distance QCD effects correcting the LR Model contributions to meson-mixing observables at the Next-to-Leading Order. I then revisit a simple realization of LR Models, containing doublet scalars, and combine in a global fit electroweak precision observables, direct searches of the new gauge bosons and meson oscillation observables, a task performed within the \texttt{CKMfitter} statistical framework. Finally, I also cover a different issue, namely the modeling of theoretical uncertainties, a class of uncertainties specially important for flavour physics. Different frequentist schemes are compared, and their differences are illustrated with flavour-oriented examples.}
%
\end{center}

\thispagestyle{empty}

\clearpage
\setcounter{page}{1}

%PhD thesis submitted to Univ. Paris-Sud, Universit\'{e} Paris-Saclay. Advisors: S. Descotes-Genon and V. Bernard. Includes results from hep-ph/1501.05483, hep-ph/1512.00543, hep-ph/1611.04768.

==> Diagrams_contributing_v3.tex <==
\section{Contributions to meson-mixing}\label{sec:DiagramsSMLRM}

Formally, from the Lagrangian $ \mathcal{L} $ of the theory one builds all the possible contributions to the meson-mixing amplitude from the generating Green's function, $ \langle {\rm \mathbf{T}} \exp \left[ i \int d^4 x \, \mathcal{L} (x) \right] \rangle_{\vert \Delta F \vert = 2} $. We aim at keeping the set of diagrams compatible with gauge invariance at first order in

\begin{equation}
\beta = M^2_W / M^2_{W'} = \mathcal{O} (\epsilon^2) \, .
\end{equation}
Apart from the $ W W $ box already found in the SM, one important class of contributions includes the exchange of a single $ W' $ in a box together with a $ W $, which turns out not to be gauge invariant by itself. The set of diagrams necessary for the gauge invariance of the $ W W' $ box includes loop corrections of the Higgs self-energy and Higgs $ \vert \Delta F \vert = 1 $ coupling \cite{Basecq:1985cr} \cite{Hou:1985ur}. The other classes of diagrams we consider consist of charged Higgs and tree level neutral Higgs exchanges, cf. Figure~\ref{fig:tabNPdiagrams}.

\subsection{SM}

\begin{figure}
	\centering
		\SetWidth{1.2}
		\vspace{-2cm} \begin{picture}(125,115)(-10,0)
		\ArrowLine(40,80)(0,115)
		\Text(0,100)[t]{$ s $}
		\ArrowLine(0,0)(40,35)
		\Text(0,28)[t]{$ d $}
		\ArrowLine(85,80)(40,80)
		\Photon(40,80)(40,35){4}{8}
		\ArrowLine(125,115)(85,80)
		\Text(120,104)[t]{$ d $}
		\ArrowLine(85,35)(125,0)
		\Text(120,24)[t]{$ s $}
		\ArrowLine(40,35)(85,35)
		\Photon(85,80)(85,35){4}{8}
		\Text(60,95)[t]{$ u, c, t $}
		\Text(60,28)[t]{$ u, c, t $}
		\Text(18,60)[t]{$W$}
		\Text(102,60)[t]{$W$}
		\Text(70,-20)[]{(a)}
		\end{picture}
		\vspace{2cm} \input{Meson_mixing_diagrams.tex}
\caption{Figure (a): contribution already found in the SM. Figures (b)-(f): set of diagrams giving the main new contributions to kaon mixing in Left-Right Models. The set (b), (c), (d) and a contribution from (e), tree level neutral Higgs exchanges, forms a gauge invariant set of diagrams. Another important class of new contributions includes charged Higgs exchanges in a box, diagram (f). Instead of the neutral $ \mathcal{CP}- $even Higgs $ H^0_1 $, we could consider as well the $ \mathcal{CP}- $odd one, $ A^0_1 $. Diagrams where the $ W $ and $ W' $ are replaced by their respective Goldstone bosons have also to be taken into account.}\label{fig:tabNPdiagrams}
\end{figure}

In the SM, the only contribution we have is shown in Figure~\ref{fig:tabNPdiagrams} (a), where two $ W $ bosons are exchanged and the internal flavours can be $ u, c, t $. Of course, the full set of diagrams also includes the exchange of the corresponding Goldstone boson $ G $ instead of $ W $, i.e. $ W G $ and $ G G $ boxes. We note that the set of diagrams is gauge invariant by itself, and that it is finite (no renormalization is needed at this stage). The final expression is found for instance in \cite{Buchalla:1995vs}, and is given by

\begin{eqnarray}\label{eq:SMbox}
H^{\rm SM} &=&\frac{G_F^2 M^2_W}{4\pi^2} Q^{VLL} \sum_{U,V=u,c,t}\lambda_U^{LL}\lambda_V^{LL} \\
& \times & [(1+x_U x_V / 4)I_2(x_U,x_V)-2 x_U x_V I_1(x_U,x_V)]\, + h.c. ,
\nonumber
\end{eqnarray}
\noindent
where the operator $ Q^{VLL} $ is

\begin{equation}
Q^{VLL} = \bar{d} \gamma^\mu P_L s \cdot \bar{d} \gamma_\mu P_L s \, .
\end{equation}
The combinations of CKM matrix elements are given by

\begin{equation}
\lambda^{AB}_U = V^{A *}_{U q_1} V^{B}_{U q_2}
\end{equation}
($ q_{1,2} $ are the external flavours) and $ I_{1,2} (x_U, x_V) $ are the Inami-Lim functions \cite{Inami:1980fz}

\begin{eqnarray}\label{eq:InamiLimSMcase}
I_1 (x_U,x_V) & = & \frac{x_U\log x_U}{(1-x_U)(x_U-x_V)} + (U\leftrightarrow V) , \nonumber\\
I_2 (x_U,x_V) & = & \frac{x_U^2\log x_U}{(1-x_U)(x_U-x_V)} + (U\leftrightarrow V) \, .
\end{eqnarray}

We further apply the unitarity of the CKM matrix, i.e. $ \sum_{U=u,c,t} \lambda^{LL}_U = 0 $, to rewrite Eq.~(\ref{eq:SMbox}) under a different form

\begin{eqnarray}\label{eq:SMboxUnitarity}
&& H^{\rm SM} = \frac{G_F^2 M_W^2}{4 \pi^2}
\Bigg[ \lambda_c^{LL} \lambda_c^{LL} S^{LL}(x_c) \\
&& + \lambda_t^{LL} \lambda_t^{LL} S^{LL}(x_t) +2 \lambda_t^{LL} \lambda_c^{LL} S^{LL}(x_c,x_t) \Bigg] Q^{VLL} + h.c. , \nonumber
\end{eqnarray}
where we have defined the following \textit{loop functions}

\begin{eqnarray}\label{eq:SMloopfunctions}
S^{LL}(x_c)&=& x_c+ {\cal O}(x_c^2)\,,\\
S^{LL}(x_t)&=&x_t\biggl(\frac{1}{4}+\frac{9}{4}\frac{1}{1-x_t}
-\frac{3}{2}\frac{1}{(1-x_t)^2}\biggr) -\frac{3}{2}\biggl(\frac{x_t}{1-x_t}
 \biggr)^3 \log x_t \,,
\nonumber \\
S^{LL}(x_c,x_t)&=& -x_c \log x_c+ x_c F(x_t)+ {\cal O}(x_c^2 \log x_c)  \, , \nonumber
\end{eqnarray}
with

\begin{equation}
F(x_t)=\frac{x_t^2 - 8 x_t +4}{4(1-x_t)^2} \log x_t +\frac{3}{4} \frac{x_t}{(x_t-1)} \, .
\end{equation}

We refer to the above three contributions as charm-charm, top-top and charm-top respectively, which are proportional to $ \lambda^{LL}_U \lambda^{LL}_V $, $ U, V = c, t $. Note that, thanks to the unitarity of the CKM matrix, $ \mathcal{O} (\log x_c) $ in the charm-charm contribution vanishes, while due to the different masses in the charm-top case this factor is present.

\subsection{LRM}

We start by discussing the contributions from box diagrams. Due to the $ W, W' $ mixing, which modifies the structure of the $ W $ coupling at order $ \epsilon^2 $ by the introduction of right-handed couplings, we reconsider the SM-like $ W W $ box which is also present in the LRM. Then, since right-handed couplings are also present, we distinguish the following cases: zero, one, two, three and four right-handed couplings. Each time there is a right-handed coupling, the whole contribution gets suppressed by $ \epsilon^{2} $, and the combination of a left-handed coupling with a right-handed one implies a chiral flip of the intermediate up-type quark. Now, diagrams with an odd number of chirality flips give no contribution when the momenta of the external quarks are set to zero, since the integral on the loop momentum is odd. Therefore, we consider only the left-handed coupling of the $ W $, since the next contribution involving two right-handed couplings is suppressed by $ \epsilon^4 $, thus implying that $ W W $ box in LRM has the same expressions found in the SM, Eqs.~\eqref{eq:SMboxUnitarity}-\eqref{eq:SMloopfunctions}.

Apart from the $ W W $ box, we also have $ W W' $ boxes. The heavy character of the $ W' $ implies that we need to consider only its right-handed coupling. The $ WW' $ box diagrams are usually calculated in the \tHF gauge ($ \xi_{W,W'} = 1 $), see e.g. \cite{Ecker:1985vv}, and we have

\begin{eqnarray}\label{eq:boxWWprimePrevious}
A^{({\rm box})} &=&\frac{G_F^2 M^2_W}{4\pi^2} 2 \beta h^2 \langle Q_2^{LR} \rangle \sum_{U,V=u,c,t}\lambda_U^{LR}\lambda_V^{RL} \sqrt{x_Ux_V} \\
& \times & [(4+x_Ux_V \beta)I_1(x_U,x_V,\beta)-(1+\beta)I_2(x_U,x_V,\beta)] \,,
\nonumber
\end{eqnarray}
\noindent
where the operator $ Q^{LR}_{2} $ is

\begin{equation}
Q^{LR}_{2} = \bar{d} P_R s \cdot \bar{d} P_L s \, .
\end{equation}
Note that this operator has a very different structure when compared to the SM operator, $ Q^{VLL} $.

In Eq.~\eqref{eq:boxWWprimePrevious}, gauge couplings are contained in $ h = g_R / g_L $, and

\begin{eqnarray}\label{eq:InamiLimObetaLRM}
I_1 (x_U,x_V,\beta) & = & \frac{x_U\log x_U}{(1-x_U)(x_U-x_V)} + (U\leftrightarrow V) + \mathcal{O}(\beta) , \\
I_2 (x_U,x_V,\beta) & = & \frac{x_U^2\log x_U}{(1-x_U)(x_U-x_V)} + (U\leftrightarrow V) - \log\beta + \mathcal{O}(\beta) \, , \nonumber
\end{eqnarray}
(corrections in $ \beta $ are found for example in \cite{Ecker:1985vv}). In the \tHF gauge, the contributions to $ A^{({\rm box})} $ seen in the second line of Eq.~\eqref{eq:boxWWprimePrevious} come from the four following diagrams:

\begin{itemize}
	\item $ WW' \Rightarrow I_1(x_U,x_V,\beta) $ term, \\
	\item $ GW' \Rightarrow I_2(x_U,x_V,\beta) $ term, \\
	\item $ WG' \Rightarrow \beta I_2(x_U,x_V,\beta) $ term, of higher order in $ \beta $, and \\
	\item $ GG' \Rightarrow x_U x_V \beta I_1(x_U,x_V,\beta) $ term, also of higher order in $ \beta $, \\
\end{itemize}
where $ G $ ($ G' $) is the Goldstone boson associated to the light (heavy) gauge boson $ W $ ($ W' $). The different handednesses of the main couplings of the $ W, W' $ imply chiral flips leading to the overall mass term, seen in the first line of Eq.~\eqref{eq:boxWWprimePrevious}. Note that due to the overall mass factors, diagrams involving an up-quark are very much suppressed and can be ignored. Expanding $ A^{({\rm box})} $ in $ \beta = M^{2}_{W}/M^{2}_{W'} $ and $ x_c = m^{2}_{c}/M^{2}_{W} $ one has

\begin{eqnarray}\label{eq:boxWWprime}
A^{({\rm box})} &=& \frac{G_F^2 M_W^2}{4 \pi^2} 2 \beta h^2 \langle Q_2^{LR} \rangle \biggl[ \lambda_c^{LR}\lambda_c^{RL}S^{({\rm box})}(x_c, x_c, \beta) \\
& + & \lambda_t^{LR}\lambda_t^{RL}S^{({\rm box})}(x_t, x_t, \beta)+  (\lambda_c^{LR}\lambda_t^{RL}+\lambda_t^{LR}\lambda_c^{RL})S^{({\rm box})}(x_c, x_t, \beta)\biggr]\,,\nonumber
\end{eqnarray}
where the loop functions are

\begin{eqnarray}
S^{({\rm box})} (x_c, x_t, \beta) \!\!&=& \!\! \sqrt{x_c x_t}\left[\frac{x_t - 4}{x_t - 1} \log (x_t) + \log (\beta) \right] + \mathcal{O} (\beta, x^{3/2}_c)\,, \\
S^{({\rm box})} (x_t, x_t, \beta) \!\!&=&\!\! x_t\left( \frac{x_t^2 - 2 x_t + 4}{(x_t - 1)^2} \log (x_t) + \frac{x_t - 4}{x_t - 1} + \log (\beta) \right) + \mathcal{O} (\beta)\,, \nonumber\\
&& \\
S^{({\rm box})} (x_c, x_c, \beta) \!\!&=&\!\! x_c  \left( 4 \log (x_c) + 4 + \log (\beta) \right) + \mathcal{O} (\beta, x^2_c)\,. \label{eq:boxWWprimecc}
\end{eqnarray}

The question of gauge invariance has been addressed in several papers \cite{Basecq:1985cr} \cite{Hou:1985ur} \cite{Kenmoku:1987fm} \cite{GagyiPalffy:1997hh}. It has been shown in \cite{Kenmoku:1987fm} that the $ W W' $ box diagram forms a gauge invariant set only if neutral Higgs exchanges imply no FCNC at tree level. However, we have seen that this is not the case in the class of LR Models we are considering, cf. Section~\ref{sec:couplingsHfermionsLRM}. The required diagrams for gauge invariance are shown in Figure~\ref{fig:tabNPdiagrams} (c, d). Note that, in order to be consistent with the order of these four point Green's functions, we should consider the renormalization of the Higgs mass and couplings. However, by considering on-shell subtractions as described in \cite{Basecq:1985cr} the bare values are equal to the renormalized ones.

Below, we give the expressions of the vertex and self-energy diagrams in the \tHF gauge. They have been explicitly calculated in \cite{Bertolini:2014sua}, for instance, and depend on the Higgs mass through $ \omega_i = M^2_{W'} / M^2_{H_i} $:

\begin{eqnarray}\label{eq:selfWWprime}
A^{\rm (self)} =
-2\beta \sum^2_{i=1} \mathcal{F}^2_i \omega_i h^2\frac{G_F^2 M_W^2}{4\pi^2}  \langle Q_2^{LR}\rangle S_S(\omega_i) \sum_{U,V=c,t} \lambda_U^{LR}\lambda_V^{RL}  \sqrt{x_U x_V} \,,
\end{eqnarray}

\begin{eqnarray}
S_S(\omega) = -2+\frac{(1-\omega^2)}{\omega}\log\left|\frac{1-\omega}{\omega}\right| +\mathcal{O}(\beta)\,, \nonumber\\
\end{eqnarray}
and

\begin{equation}\label{eq:vertexWWprime}
A^{\rm (vertex)} =
-32\beta \sum^2_{i=1} \mathcal{F}_i \omega_i h^2\frac{G_F^2 M_W^2}{4\pi^2} \langle Q_2^{LR}\rangle S_V(\omega_i)  \sum_{U,V=c,t} \lambda_U^{LR}\lambda_V^{RL}  \sqrt{x_U x_V} \,,
\end{equation}

\begin{equation}
S_V(\omega) = -1+(1-\omega)\log\left|\frac{1-\omega}{\omega}\right| + \mathcal{O}(\beta^{1/2}) \, ,
\end{equation}

The above expressions include a $ \mathcal{CP}- $even and a $ \mathcal{CP}- $odd Higgs. Note that the mixed propagator of a $ \mathcal{CP}- $even and a $ \mathcal{CP}- $odd Higgs gives no contribution, due to their real and pure imaginary couplings, respectively.

The functions $ \mathcal{F}_i = k F_i G_i $ correct the limiting case $ w \rightarrow 0^+ $, and are calculated from the corrections to the couplings of the scalar sector to the gauge bosons (proportional to $ F_i $) and quarks (proportional to $ G_i $) when $ w \neq 0 $. Their expressions are given by

\begin{eqnarray}
\mathcal{F}_1  &=&\frac{1}{ 2  (1 - r^2)(1 + \beta(x) w^2) (1 - \delta^2)} 
 \biggl( \bigl(-k^2  + (k^2 -2(1 +  \nu(x) )) X \bigr) (1+ \delta^2) \biggr.
\nonumber \\
&&\biggl.+2 \bigl(1 + \nu(x) + \bigl(r^2 -\beta(x) w^2 (1 - r^2)  +  \nu(x)\bigr) \delta^2 \bigr) \biggr)
\end{eqnarray}
while $ \mathcal{F}_2 = 1 - \mathcal{F}_1 $ is calculated from $ \mathcal{F}_1 $ by changing $\delta \to 1/\delta$, where $\delta=M_{H_2}/M_{H_1}$ is the ratio of the mass of the scalars $ H_2, A_2 $ over the one of the scalars $ H_1, A_1 $. The other functions seen in the expression of $ \mathcal{F}_i $ are

\begin{eqnarray}
&& X=\sqrt{1- \frac{4 \delta^2}{(1+ \delta^2)^2} \frac{\left(1+r^2\right)\left(1+ \beta(x) w^2\right)}{k^2}} \, , \nonumber\\
&& \beta(x)=(1+x^2)/(1+r x)^2  \, , \quad \quad \nu(x) = w^2/(1+ r x ) \, , \\
&& k^2 = 1 + r^2 + w^2 \, . \nonumber
\end{eqnarray}
In the above expressions, we have indicated the dependence on the parameter $ x $ defined as $x=\mu'_1 /\mu'_2$, which is the ratio of the two trilinear coupling constants seen in the scalar potential in Eq. XXX. Its origin amounts to the diagonalization of the mass matrix in the scalar sector, calculated at the minimum of the scalar potential. It is easy to verify that $ \mathcal{F}_2 \rightarrow 0 $ when $ w \rightarrow 0^+ $, by using the fact that the ratio of masses $ \delta $ goes to infinity due to $ M^2_2 \propto w^{-1} $. Therefore, in this limiting case the second set of scalars $ H_2, A_2 $ decouples from the phenomenology under study here.

The remaining contribution necessary for gauge invariance comes from a tree level diagram, cf. Figure~\ref{fig:tabNPdiagrams} (e). It originates from the mixing between $ A^{0}_{1} $ and $ A^{0}_{2} $, or between $ H^{0}_{1} $ and $ H^{0}_{2} $, through $ W W' $ loops leading to a gauge dependence of the scalar couplings, just like the diagram in Figure~\ref{fig:tabNPdiagrams} (d) is not gauge invariant by itself. We give in the following expression both the gauge independent (first line) and the gauge dependent (second line) contributions from the tree level diagram in the \tHF gauge:

\begin{eqnarray}\label{eq:allTheTreeLevelContributions}
A^{(H^0)} &=& \biggl( - \frac{4 G_F \beta u}{\sqrt{2}} \frac{k^2}{1+r^2} \sum^2_{i=1} \omega_i \tilde G_i^2 \nonumber\\
&& + h^2 \frac{G_F^2 M_W^2}{2 \pi^2} \beta {\cal F}^r \sqrt{\omega_1 \omega_2}   S_S\bigl(\sqrt{\omega_1 \omega_2}\bigr) \biggr) \\
&& \sum_{U, V=c, t} \lambda_U^{LR}\lambda_V^{RL} \sqrt{x_U x_V} \langle Q_2^{LR}\rangle \, , \nonumber
\end{eqnarray}
where $u=(1+r^2)^2/(1-r^2)^2$. The function $ \mathcal{F}^r $ is defined from $ \mathcal{F}^r = \sum^2_{i=1} \mathcal{F}^2_i - 1 $, where $ \mathcal{F}_i $ is found in Eq. XXX. One can check that the gauge dependent part of the above expression goes to zero like $ r w^3 $ when $ w $ goes to zero. The full discussion concerning gauge invariance in the general case where $ w \neq 0 $ is found in reference \cite{Bernard}.

The function $ \tilde G_i^2 $ seen in the gauge independent part is calculated from $\tilde G_i^2= (1+r^2) G_i^2/u$ where $ G_i $ corrects the couplings of the scalars to the quarks when $ w \neq 0 $.  Its expression is given by

\begin{equation}
\tilde G_2^2=\frac{k^2(1- \delta^2  ( 1 -\left(1+1/\delta^2\right)X)) -2w^2(1-\beta(x)(1+r^2))}{2 (1-\delta^2)
(1+r^2)  (1+ \beta(x) w^2) } \, ,
\end{equation}
while $ \tilde G_1^2 $ is determined from the relation $\tilde G_1^2=1- \tilde G_2^2$.

Note that contributions proportional to $ \bar{s} P_L d \cdot \bar{s} P_L d $ or $ \bar{s} P_R d \cdot \bar{s} P_R d $ come at a higher order: once all the tree level Higgs contributions are considered, i.e. $ \mathcal{CP}- $even and $ \mathcal{CP}- $odd ones, they cancel each other since they have degenerate masses at leading order in $ \mathcal{O} (\epsilon^0) $, see Appendix XXX.

Apart from the contributions given in Eqs.~\eqref{eq:SMboxUnitarity}, \eqref{eq:boxWWprime}, \eqref{eq:selfWWprime}, \eqref{eq:vertexWWprime}, \eqref{eq:allTheTreeLevelContributions}, the last set of diagrams, shown in Figure~\ref{fig:tabNPdiagrams} (f) consists of boxes $ W H^{\pm}_1 $ and $ G H^{\pm}_1 $, where $ H^{\pm}_1 $ is a heavy, electrically charged Higgs which couples as $ G' $, cf. Table XXX. As discussed in \cite{GagyiPalffy:1997hh}, it alone does not form a gauge invariant set, but the other diagrams necessary for gauge invariance (vertex and self-energy diagrams) contribute at a higher order in $ \beta $ in the \tHF gauge. In this case, we have

\begin{eqnarray}
H^{(H^{\pm} \, {\rm box})} &=&\frac{G_F^2 M^2_W}{4\pi^2} \frac{k^2}{1+r^2} Q_2^{LR} \sum^2_{i=1} \tilde{G}^2_i 2 \omega_i \beta u (1 - \beta) \sum_{U,V=u,c,t}\lambda_U^{LR} \lambda_V^{RL} \sqrt{x_U x_V} \nonumber\\
& \times & [-I_2(x_U,x_V,\omega_i \beta)+x_U x_V I_1(x_U,x_V,\omega_i \beta)]\, + h.c. \, ,
\end{eqnarray}
\noindent
or, expanding in $ \beta $ and $ x_c $,

\begin{eqnarray}\label{eq:chargedHiggsContribution}
H^{(H^{\pm} \, {\rm box})} &=&
 \frac{G_F^2 M_W^2}{4\pi^2} \frac{k^2}{1+r^2} Q_2^{LR} \sum^2_{i=1} \tilde{G}^2_i 2 \omega_i \beta u \sum_{U,V=c,t} \lambda_U^{LR}\lambda_V^{RL} \nonumber\\
&& \quad \sqrt{x_U x_V} S^H_{LR}(x_U,x_V, \beta \omega_i)\, + h.c. \, ,
\end{eqnarray}
with

\begin{eqnarray}\label{eq:loopFunctionsBoxH}
S^H_{LR} (x_c, x_t, \omega \beta) &=& \left( \frac{x_t}{x_t - 1} \log (x_t) + \log (\omega \beta) \right) + \beta \cdot \mathcal{O} (\beta, x_c) , \\
S^H_{LR} (x_t, x_t, \omega \beta) &=& \left( \frac{2 x_t}{x_t - 1} \log (x_t) - x_t + \log (\omega \beta) \right) + \mathcal{O} (\beta^2), \\
S^H_{LR} (x_c, x_c, \omega \beta) &=& \log (\omega \beta) + \beta \cdot \mathcal{O} (\beta, x_c) .
\end{eqnarray}
